Review and prospects of hot exozodiacal dust research for future exo-Earth direct imaging missions

Hot exozodiacal dust is dust in the innermost regions of planetary systems, at temperatures around 1000K to 2000K, and commonly detected by near-infrared interferometry. The phenomenon is poorly understood and has received renewed attention as a potential risk to a planned future space mission to image potentially habitable exoplanets and characterize their atmospheres (exo-Earth imaging) such as the Habitable Worlds Observatory (HWO). In this article, we review the current understanding of hot exozodiacal dust and its implications for HWO. We argue that the observational evidence suggests that the phenomenon is most likely real and indeed caused by hot dust, although conclusive proof in particular of the latter statement is still missing. Furthermore, we find that there exists as of yet no single model that is able to successfully explain the presence of the dust. We find that it is plausible and not unlikely that large amounts of hot exozodiacal dust in a system will critically limit the sensitivity of exo-Earth imaging observations around that star. It is thus crucial to better understood the phenomenon in order to be able to evaluate the actual impact on such a mission, and current and near-future observational opportunities for acquiring the required data exist. At the same time, hot exozodiacal dust (and warm exozodiacal dust closer to a system's habitable zone) has the potential to provide important context for HWO observations of rocky, HZ planets, constraining the environment in which these planets exist and hence to determine why a detected planet may be capable to sustain life or not.

==> sections/executive_summary.tex <==
[Note by Steve:  Use this for the report, but not for the version developing into a refereed paper.]

Study Analysis Group (SAG)~\#23\footnote{\url{https://sites.google.com/view/sag23-exozodiacaldust/home}} ``The Impact of Exozodiacal Dust on Exoplanet Direct Imaging Surveys'' was established as part of NASA's Exoplanet Exploration Program Analysis Group (ExoPAG).  In this report from SAG~\#23 we review the current knowledge of hot exozodiacal dust and open questions, the current state of research in the field, and future prospects of improving our understanding of the dust in support of a future, large space mission to search for rocky, potentially habitable planets and to search for bio-signatures in their atmospheres through direct imaging and spatially resolved spectroscopy (exo-Earth imaging mission).

Exozodiacal dust -- or exozodi for short -- is warm dust in and near a star's habitable zone (HZ), with temperatures $\sim$300\,K, and hot dust closer in, with temperatures $\sim$1000\,K to $\sim$2000\,K.  It poses potential obstacles to an exo-Earth imaging mission because it adds noise, confusion, and coronagraphic leakage to these observations.  Understanding the properties, origin, and dynamics of the dust as a function of other, more accessible system parameters such as stellar properties or the presence of cold dust or giant planets in the system can help predict the impact of these noise sources for future mission targets.  In addition, studying the dust can give important insight into the presence of planets, planetesimals, and comets orbiting a star, and their dynamics and interactions, thereby crucially constraining the architecture and evolution of a planetary system.  This may have profound implications for whether a rocky, HZ planet is Earth-like compared to, e.g., barren or a water world.

During recent efforts to define the scope of ``precursor science'' for a large NASA flagship mission capable of an exo-Earth imaging survey, the importance of better understanding hot exozodiacal dust -- in addition to HZ dust -- was recognized.  Hot exozodi is dust closer to the star than the HZ, likely reaching as close as the dust sublimation distance (typically 4 to a few 10s of stellar radii depending on stellar luminosity and dust composition).  This dust has been detected as a $\sim$1\% near-infrared (nIR) excess around $\sim$20\% of the main-sequence stars surveyed.  The presence of hot dust around a significant fraction of stars and/or its persistence over a significant fraction of a star's lifetime are difficult to explain, however the hypothesis that the emission originates from dust is observationally well-supported.  Most recently, observations in $L$~band have shown that the excess emission is indeed consistent with blackbody emission from dust at a temperature of $\sim$1000\,K.  Furthermore, no scenario other than the presence of dust has been shown to plausibly explain the excess emission so far.

The risks to an exo-Earth imaging mission from hot exozodiacal dust are two-fold.  It is thought that the dust is supplied by material further out in the planetary system that must move through the system's HZ, potentially producing emission there that may limit our ability to detect and characterize rocky planets there.  Moreover, the hot dust produces extended and likely polarized excess emission around the star that may limit the contrast that can be reached by coronagraphic starlight suppression methods.

We conclude from our review that hot exozodiacal dust is currently not sufficiently well understood to evaluate its risk for exo-Earth imaging.  It is, however, plausible and not unlikely that large amounts of such dust in a system will critically limit the sensitivity of exo-Earth imaging observations around that star.  In particular, the location and properties of the dust are poorly known and its impact on exo-Earth imaging is poorly studied, so that the level of hot dust that would prevent exo-Earth imaging around its host star is poorly constrained.  Moreover, the fraction of stars harboring dust at various, likely relevant levels of dust is poorly constrained.  Furthermore, there is currently insufficient knowledge of the dust's origin.  Hence, predicting the presence of the dust around a given target star at any meaningful level, or the properties and amount of dust moving through the system's HZ to supply the hot dust, is impossible.  The phenomenon thus critically needs to be better understood to evaluate the actual impact on such a mission, and current and near-future observational opportunities have the strong potential to provide the required data.

